Automated Transparency: A Legal and Empirical Analysis of the Digital Services Act Transparency Database

The Digital Services Act (DSA) is a much awaited platforms liability reform in the European Union that was adopted on 1 November 2022 with the ambition to set a global example in terms of accountability and transparency. Among other obligations, the DSA emphasizes the need for online platforms to report on their content moderation decisions (`statements of reasons' - SoRs), which is a novel transparency mechanism we refer to as automated transparency in this study. SoRs are currently made available in the DSA Transparency Database, launched by the European Commission in September 2023. The DSA Transparency Database marks a historical achievement in platform governance, and allows investigations about the actual transparency gains, both at structure level as well as at the level of platform compliance. This study aims to understand whether the Transparency Database helps the DSA to live up to its transparency promises. We use legal and empirical arguments to show that while there are some transparency gains, compliance remains problematic, as the current database structure allows for a lot of discretion from platforms in terms of transparency practices. In our empirical study, we analyze a representative sample of the Transparency Database (131m SoRs) submitted in November 2023, to characterise and evaluate platform content moderation practices.

==> leftovers.tex <==



\subsection{Missing Information}
In this section, we identify the attributes which are either completely missing or overwhelmingly missing in the SoRs submitted by VLOPs.
$end\_date\_visibility\_restriction$ is having mostly NULL values suggesting the once a content is restricted, it is permanent and irreversible.
VLOPs are not making monetary restrictions because the $decision\_monetary$ attribute is almost NULL. Provision of service ($decision\_provision$), which would have values whether content is partially or totally suspended, is another attribute that is not being populated. VLOPs are specifying the grounds on which decisions are made through the $decision\_ground$ attribute, however, detailed reasons are missing in most of the cases since the attribute $decision\_ground\_reference\_url$ is mostly unpopulated. 
In similar lines, the attribute $category$ does indicate different types of violations but the attribute $category\_specification$ is missing values. 

\subsection{Generic Non-Meaningful Information}
VLOPs submit generic templates particularly in free text attributes designed in DTD, namely, $decision\_facts$, $illegal\_content\_explanation$, and $incompatible\_content\_explanation$. 
Although filling some information does comply with DSA provision but it does not address the objective of transparency because the submitted information is not meaningful.




\subsection{Data Collection - Sampling Strategy}

Prior to the launch of daily dumps, we collected SoRs data submitted at DTD by the VLOPs using different sampling strategies.
At the time of launch, DTD had a limitation in the amount of SoRs that can be downloaded from DSA website. 
Only the most recent 10K SoRs were available for download which were spread across 200 pages, each listing 50 SoRs. 
Out of these 10K SoRs, the top 1K was available for download as CSV file.
During this phase, we collected a \emph{sample} of 10,080,879 SoRs during 25 September, 2023 to 25 October, 2023. 
We started the live data collection process in first week of October, 2023. Consequently, the data already pushed into DTD was no longer available on the DTD website. So, we adopted two approaches for sample data collection, one for collecting older data during 25 September - 5 October, 2023 and another for collecting live data from 6 October 2023 onwards. 

\begin{itemize}
\item Old sample data (25 Sept - 5 Oct, 2023): Initially, we explored the Internet old archive which caches snapshots of website pages on earlier dates. 
However, it turned out that all 200 pages at older days were not being cached. So, we leverage the `advanced search' option of DTD website and collect \textbf{998,524 SoRs} during this period of 25 Sept to 5 Oct by performing platform-wise and day-wise search queries. 

\item Live sample data (6 Oct onwards): From 6 October onwards, we collect SoRs by periodic pulling for at least 6 hrs each day at different times in the day.
If the pull interval is large, we would loose data because SMPs are pushing at faster rate than what we are pulling. 
If the pull interval is small, we get a lot of duplicate SoRs. 
So, after trying different pull intervals, we find pull interval of 60 seconds most optimal.
In each pull request made per minute, we would get up to 1K (single csv file) SoRs from the DTD. Following this approach, we obtain 9,082,355 SoRs during the period of 6 - 25 October, 2023.
Data collected so far is summarized in Table \ref{tab:sample_data_stats} which also shows day-wise SoRs collected along with timestamps of the day when SoRs got added into DTD. 
%We observe that we collect 9.8\% of the total 31,275,032 SoRs pushed into DTD.
\end{itemize}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
         Day & Time of the day & \#SoRs collected & \#SoRs pushed\\
         \hline
         \multicolumn{4}{c}{Old Sample Data Collection} \\
         \hline
         2023-09-25 & ... & 55,195 & 1,771,586 \\
         2023-09-26 & ... & 104,406 & 3,119,735 \\
         2023-09-27 & ... & 110,327 & 3,788,840 \\
         2023-09-28 & ... & 93,616 & 3,540,728 \\
         2023-09-29 & ... & 98,469 & 3,396,397 \\
         2023-09-30 & ... & 93,343 & 3,810,673 \\
         2023-10-01 & ... & 91,579 & 3,534,355 \\
         2023-10-02 & ... & 87,958 & 3,702,367 \\
         2023-10-03 & ... & 106,545 & 3,730,492 \\
         2023-10-04 & ... & 85,506 & 3,475,957 \\
         2023-10-05 & ... & 71,580 & 5,511,060 \\
         \hline
         \multicolumn{4}{c}{Live Sample Data Collection} \\
         \hline
         2023-10-06 & 0150 - 1350 hrs & 382,681 & 5,489,407 \\
         2023-10-07 & 0753 - 1443 hrs & 361,000 & 3,776,492 \\
         2023-10-08 & 0744 - 2141 hrs & 716,000 & 4,618,013 \\
         2023-10-09 & 0731 - 1946 hrs & 568,668 & 4,328,084 \\ 
         2023-10-10 & 0702 - 1351 hrs & 345,000 & 3,958,082 \\
         2023-10-11 & 0656 - 1343 hrs & 355,000 & 4,510,184 \\
         2023-10-12 & 0713 - 1357 hrs & 353,000 & 4,594,770 \\
         2023-10-13 & ... & 346,000 &	4,637,821 \\
2023-10-14 & ... & 346,000 & 5,232,892 \\
2023-10-15 & ... & 695,894 &	4,488,693 \\
2023-10-16 & ... & 598,684 & 4,285,577 \\
2023-10-17 & ... & 837,079 & 14,286,003 \\
2023-10-18 & ... & 122,854 & 61,650,478 \\
2023-10-19 & ... & 136,043 &	30,752,091 \\
2023-10-20 & ... & 539,898 & 7,189,213 \\
2023-10-21 & ... & 933,000 & 6,712,728 \\
2023-10-22 & ... & 845,000 &	6,718,233 \\
2023-10-23 & ... & 600,554 & 7,153,654 \\
2023-10-24 & ... & ... & ... \\
2023-10-25 & ... & ... & ... \\
         \hline
         \multicolumn{2}{c|} {Total} & 	&  \\
    \end{tabular}
    \caption{Sample Data Collection Day-wise Statistics.}
    \label{tab:sample_data_stats}
\end{table}



\section{Future Directions}
\begin{itemize}
\item Text analysis on SoRs:
There are attributes in the SoRs schema design, namely, $decision\_facts$, $incompatible\_content\_explanation$, and $illegal\_content\_explanation$ that provides a provision for VLOPs to provide more information (free text) on the reasons, facts, and circumstances for moderation of content, thereby, enhancing transparency. While most platforms provide a standard generic templates but some VLOPs like AliExpress provide details reasons, particularly for the intellectual property rights infringements which needs to be studied further in detail. 

\item Territorial jurisdictions:
While most of the content moderation happens across EU region, there are still a large number of SoRs specifying a particular country as territorial scope for the moderation decisions. 
This needs furhter investigation to understand distribution of country specific SoRs, linkages of such SoRs with national laws, and types of violations that are reported specific to countries.

\item Correlational analysis:
Most of our analysis are on single attribute. It would be interesting to study and analyze the interplay between different attributes. 
For instance, is there a correlation between the delay in moderation and uploads with respect to fraction of automated detection and decision, type of content, and type of violation category. 
Likewise, is there a dependency between the facts and circumstances relied upon and type of restriction applied. 

\item Learning based models:
It would be interesting to build models to predict delay, understand factors that contribute to the delay in moderation and upload to DTD by VLOPs. 
Further, based on the submission behavior of different VLOPs, they can be clustered using unsupervised learning models.

\item Comparison with transparency reports:
VLOPs are also required to submit transparency reports which provide aggregate view of the moderation decisions undertaken by them. 
It would be interesting to compare the SoRs submitted by VLOPs and the transparency reports during the same time frames to check for consistencies in reporting by VLOPs.

\rknote{To add some points to other stakeholders related to (1) improvements in the DSA law itself (2) improvements in design of DTD, for instance, making some attributes mandatory, so that clear and specific SoRs are submitted by VLOPs (3) mechanism to be put in place by the Commission to scrutinize SoRs submitted by VLOPs}

\end{itemize}



\textbf{List of questions based on Art 17 and 24 - compliance}
\begin{itemize}
    \item Is content deemed illegal, or incompatible with ToS? 
    \item If content is illegal, are there any specific provisions and interpretations mentioned? Same for incompatible ToS content.
    \item How often do SORs refer to community guidelines, terms of service agreements, terms and conditions etc. 
    \item What kind of restrictions are platforms imposing?
    \item Under facts and circumstances - is the identity of the notifier mentioned where relevant? 
    \item Is there any reference about clear and user-friendly information on the possibilities for redress? \ainote{should this be submitted with an SOR or rather somewhere on the platform's website?}
    \item Are SoRs uploaded "without undue delay"? What's the avg time between detection - moderation decision - upload to database?
\end{itemize}

\textbf{List of additional questions}
\begin{itemize}
    \item What are self-standing categories and what is the average length of input in those categories.
    \item What is the text similarity within platforms for SORs? What does longer text tell us as opposed to shorter text?
    \item How many attributes are overall free form and how many limited? Out of the free form, what are the limitations, and where do platforms fit in that range?
\end{itemize}

\ainote{do we want to add this set of questions?} \textbf{Differentiation in reporting behavior of the platforms}
\begin{itemize}
    \item which platforms report most SORs?
    \item which platforms report most detailed information w.r.t. facts and circumstances that led to moderation decision ($decision\_facts$)? 
    \begin{itemize}
        \item AliExpress vs Amazon vs Google Shopping: E.g., AlliExpress reports copyright violations with product ID and companies whose copyrights are violated. Amazon has same information expressed in different forms (e.g., with or without period).
        \item Facebook vs Snapchat vs Instagram: Facebook has only two categories. Perhaps we should compare platforms with similar applications with each others (e.g., Google Shopping with AlliExpress and Amazon; AppStore with GooglePlay; Instagram, TikTok, Facebook, X, SnapChat;
    \end{itemize}
     \item which platforms report most detailed information w.r.t. type of incompatible content ($incompatible\_content\_grounds$)?
     \begin{itemize}
         \item Facebook mentions only `This was a violation of "sections 3.2" of our terms of service' standard template for all SoRs. Likewise Instagram mentions only `This was a violation of  How You Can`t Use Instagram section' in all SoRs submitted.
         \item 
     \end{itemize}
     \item Detailed analysis on some platforms SoRs which are reporting more details.
     eg. Amazon reports detailed URLs in $incompatible\_content\_grounds$ and AliExpress reports details of IPR violations in $decision\_facts$.
     \item Comparing platforms \textit{group-wise} based on  similar service (Google Shopping, AliExpress, Amazon) and have similar ownership/policies (Fb Insta)
    Under content type other, where is text freeflow max 500 characters
    Platform practices
\end{itemize}

\begin{table}[!h]
    \centering
    \begin{tabular}{c|c}
         Day & \#SoRs submitted \\
        \hline
            2023-11-19  &  13,485,498 \\
            2023-11-20  &  11,321,975 \\
            2023-11-21  &  17,677,806 \\
            2023-11-22  &  13,754,557 \\
            2023-11-23  &  12,714,490 \\
            2023-11-24  &  12,400,540 \\
            2023-11-25  &  12,938,366 \\
            2023-11-26  &  12,367,133 \\
            2023-11-27  & 11,423,968 \\
            2023-11-28  &  13,038,149 \\
            \hline
            Total & 131,122,482 \\
        \hline
    \end{tabular}
    \caption{Daily Dumps Data Collection Day-wise Statistics.}
    \label{tab:daily_data_stats}
\end{table}






\section{Does transparency really work?}

RQ4: Does the DSA deliver on its transparency promises?

\rknote{Catalina and Jacob, please review, just wrote what I could understand from our last meeting's discussions, it's not complete.}

In this section, we validate at the level of DSA Transparency Database (DTD) designed by the Commission, whether it is compliant with the DSA provisions in Article 17 and 24(5).
Table \ref{tab:dsa_db_comply} specifies the provisions of the DSA Article 17 and the corresponding data attributes in the DSA Transparency Database.
While most of the provisions of DSA are taken care in the database, the provision related to the redress mechanism\footnote{Article 17(3f) says `clear and user-friendly information on the possibilities for redress available to the recipient of the service in respect of the decision, in particular, where applicable through internal complaint-handling mechanisms, out-of-court dispute settlement and judicial redress.'} is not specified in any attribute in the design of the DSA database.
\begin{table}[!h]
    \centering
    \begin{tabular}{p{7cm}|p{7cm}}
    \hline
        DSA provision(s) - excerpts & DSA Transparency Database \\
        \hline
        17(1): Providers of hosting services shall provide in SoR whether the information provided by the use is illegal content or incompatible with their terms and conditions & $decision\_ground$ attribute tells whether submitted SoR is illegal or incompatible content as per ToS of VLOP. Further, $decision\_ground\_reference\_url$ is URL to the ToS or law relied upon in taking the decision by the VLOP. \\
        \hline
        17(1): Providers of hosting services shall provide in SoRs any one of the following restrictions: (a) any restrictions of the visibility of specific items of information provided by the recipient of the service, including removal of content, disabling access to content, or demoting content;
        (b) suspension,termination or other restriction of monetary payments;
        (c) suspension or termination of the provision of the service in whole or in part;
        (d) suspension or termination of the recipient of the service's account & attributes $decision\_visibility$, $decision\_monetary$, $decision\_provision$, $decision\_account$ specify the type of restriction imposted by the VLOP. Additional attributes, namely, $decision\_visibility\_other$, $decision\_monetary\_other$, and $account\_type$ are specified to allow VLOPs to provide other related information on the restrictions. \\
    \hline
    ... & ...\\
    \hline
    ... & ...\\
    \hline
    \end{tabular}
    \caption{Mapping the DSA provisions with the attributes of the DSA Transparency Database.}
    \label{tab:dsa_db_comply}
\end{table}

\section{RQ2: Behavior of VLOPs and DSA compliance}
In this section, we characterize the behavior of VLOPs in view of DSA and also scrutinize SoRs submitted by the VLOPs to assess whether they are in compliance of DSA provisions or not.
We present our analysis on more than 131 million SoRs submitted at DTD during the ten day period during 19 - 28 November 2023 as depicted in Table \ref{tab:daily_data_stats}.
More specifically, we answer the following key questions.

\begin{itemize}
    \item Which VLOPs submit most SoRs? What are their submission rates?
    \item What are the grounds on which content is being moderated?
    \item What kind of restrictions are applied by VLOPs?
    \item What type and language of content is being moderated by VLOPs?
    \item What is the territorial scope of content moderation restrictions applied by VLOPs?
    \item What are the facts and circumstances relied upon by VLOPs in doing content moderation?
    \item What detection and decision mechanisms are being adopted by VLOPs in flagging content?
    \item What are the different categories of violation in SoRs submitted by VLOPs?
    \item Are VLOPs submitting SoRs without undue delay?
    \item How are VLOPs, similar in service and ownership, behaving in response to DSA?
\end{itemize}





\subsection{Discussion of compliance \& questions about the empirical study}
